Turning Manual Concurrent Memory Reclamation into Automatic Reference Counting

Safe memory reclamation (SMR) schemes are an essential tool for lock-free data structures and concurrent programming. However, manual SMR schemes are notoriously difficult to apply correctly, and automatic schemes, such as reference counting, have been argued for over a decade to be too slow for practical purposes. A recent wave of work has disproved this long-held notion and shown that reference counting can be as scalable as hazard pointers, one of the most common manual techniques. Despite these tremendous improvements, there remains a gap of up to 2x or more in performance between these schemes and faster manual techniques such as epoch-based reclamation (EBR). In this work, we first advance these ideas and show that in many cases, automatic reference counting can in fact be as fast as the fastest manual SMR techniques. We generalize our previous Concurrent Deferred Reference Counting (CDRC) algorithm to obtain a method for converting any standard manual SMR technique into an automatic reference counting technique with a similar performance profile. Our second contribution is extending this framework to support weak pointers, which are reference-counted pointers that automatically break pointer cycles by not contributing to the reference count, thus addressing a common weakness in reference-counted garbage collection. Our experiments with a C++-library implementation show that our automatic techniques perform in line with their manual counterparts, and that our weak pointer implementation outperforms the best known atomic weak pointer library by up to an order of magnitude on high thread counts. All together, we show that the ease of use of automatic memory management can be achieved without significant cost to practical performance or general applicability.

==> arxiv/abstract.tex <==
% !TeX root = main.tex

\begin{abstract}
Safe memory reclamation (SMR) schemes are an essential tool for lock-free data structures and concurrent programming. However, manual SMR schemes are notoriously
difficult to apply correctly, and automatic schemes, such as reference counting, have been argued for over a decade to be too slow for practical purposes. A
recent wave of work has disproved this long-held notion and shown that reference counting can be as scalable as hazard pointers, one of the most common
manual techniques. Despite these tremendous improvements, there remains a gap of up to 2x or more in performance between these schemes and faster
manual techniques such as epoch-based reclamation (EBR).

In this work, we first advance these ideas and show that in many cases, automatic reference counting can in fact be as fast as the fastest manual SMR techniques.
We generalize our previous Concurrent Deferred Reference Counting (CDRC) algorithm
% Our technique is based on the recent Concurrent Deferred Reference Counting (CDRC) algorithm of Anderson et al., which we generalize
to obtain a method for converting any standard manual SMR technique into an automatic reference counting technique with a similar performance profile.
Our second contribution is extending this framework to support weak pointers, which are reference-counted pointers that automatically break pointer cycles
by not contributing to the reference count, thus addressing a common weakness in reference-counted garbage collection.

Our experiments with a C++-library implementation show that our automatic techniques perform in line with their manual counterparts, and that our weak pointer
implementation outperforms the best known atomic weak pointer library by up to an order of magnitude on high thread counts. All together, we show that the
ease of use of automatic memory management can be achieved without significant cost to practical performance or general applicability.
\end{abstract}

==> arxiv/acquire-retire-impl.tex <==
%\section{Implementing AcquireRetire from HP, EBR, and IBR}
%\label{sec:acquire-retire-impl}



%\begin{figure}
%	\small
%	\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,linewidth=.99\columnwidth, xleftmargin=5.0ex,numbers=left]
%class AcquireRetireHP<T> {
%	using Guard = int;
%	const T* emptyhp = alloc();
%	T* hp[P][MAX_HP]; // initialized to emptyhp
%	
%	T* alloc() { return new T(); }
%	void begin_critical_section() {}
%	void end_critical_section() {}
%	void release(Guard guard) { hp[pid][guard] = emptyhp; }
%	
%	pair<T*, Guard> acquire(T** ptraddr) {
%		while(true) {
%			T* ptr = *ptraddr;
%			hp[pid][0] = ptr;
%			if(*ptraddr == ptr) return [ptr, 0]; } }
%	
%	optional<pair<T*, Guard>> try_acquire(T** ptraddr) {
%		for(int i = 1; i < MAX_HP; i++) {
%			if(hp[pid][i] == emptyhp) {
%				while(true) {
%					T* ptr = *ptraddr;
%					hp[pid][i] = ptr;
%					if(*ptraddr == ptr) return [ptr, i]; } } }
%		return @$\bot$@; }
%	
%	// retire + eject implemented as usual  };
%	\end{lstlisting}
%	\caption{\shepherd{Generalized acquire-retire implemented with hazard-pointers. We assume each process knows their process id $pid$. We introduce \op{emptyhp} to distinguish between an empty announcement slot and one that was used to announce null.}}
%	\label{fig:ar-hp}
%\end{figure}


\begin{figure}
	\small
	\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,linewidth=.99\columnwidth, xleftmargin=5.0ex,numbers=left]
class AcquireRetireEBR<T> {
	using Guard = void; // empty type, never used
	using Epoch = int;
	Epoch emptyann = INT_MAX;
	Epoch ann[P]; // initialized to emptyann
	Epoch curEpoch = 0;
	thread_local List<pair<T*, Epoch>> retired;
	
	T* alloc() { return new T(); }
	void begin_critical_section() { ann[pid] = curEpoch; }
	void end_critical_section() { ann[pid] = emptyann; }
	void release(Guard guard) {}
	
	pair<T*, Guard> acquire(T** ptraddr) { 
	  return [*ptraddr, void]; }
	
	optional<pair<T*, Guard>> try_acquire(T** ptraddr) { 
	  return [*ptraddr, void>]; }

	// retire + eject implemented as in Figure 2 of@~\cite{wen2018interval}@ };
	\end{lstlisting}
	\caption{\shepherd{Generalized acquire-retire implemented with epoch-based-reclamation. We assume each process knows their process id $pid$.}}
	\label{fig:ar-ebr}
\end{figure}


\begin{figure}
	\small
	\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,linewidth=.99\columnwidth, xleftmargin=5.0ex,numbers=left]
class AcquireRetireIBR<T> {
	using Guard = void; // empty type, never used
	using Epoch = int;
	Epoch emptyann = INT_MAX;
	Epoch beginAnn[P], endAnn[P]; // initialized to emptyann
	Epoch curEpoch = 0;
	thread_local Epoch prev_epoch = emptyann;
	thread_local int counter = 0;
	
	void begin_critical_section() { 
	  beginAnn[pid] = endAnn[pid] = prev_epoch = curEpoch; }
	void end_critical_section() { 
	  beginAnn[pid] = endAnn[pid] = emptyAnn; }
	void release(Guard guard) {}
	class Tagged<T> { Epoch birthEpoch; T t; };
	
	T* alloc() { 
		Tagged<T>* taggedObj = new Tagged<T>();
		taggedObj->birthEpoch = curEpoch;
		if(counter++ % epoch_freq == 0) curEpoch.fetch_add(1);
		return addressof(taggedObj->t); }
	
	pair<T*, Guard> acquire(T** ptraddr) { 
		while(true) {
			T* ptr = *ptraddr;
			Epoch cur_epoch = curEpoch;
			if(prev_epoch == cur_epoch) return [ptr, void];
			else endAnn[pid] = prev_epoch = cur_epoch; } }
	
	optional<pair<T*, Guard>> try_acquire(T** ptraddr) { 
		return acquire(ptraddr); }
	
	// retire + eject implemented as in@~\cite{wen2018interval}@ };
	\end{lstlisting}
	\caption{\shepherd{Generalized acquire-retire implemented with interval-based-reclamation (specifically, 2GEIBR).}}
	\label{fig:ar-ibr}
\end{figure}

==> implementation.tex <==
% !TeX root = main.tex

\section{Implementation}
\label{sec:impl}

\Hao{Info about C++ library, interface, implementation details, and possibly example usage go here. Perhaps an example usage including weak pointers should go earlier.}

\Hao{epoch\_guard automatically calls end critical section, and the Snapshot type has a destructor that automatically calls release\_snapshot.}

We plan to make our code publicly available on Github.

==> limitations.tex <==
% !TeX root = main.tex

\section{Limitations}
\label{sec:limit}

==> ref-count-impl.tex <==
\section{Implementing Concurrent Reference Counting from Generalized Acquire-Retire (pseudo-code)}
\label{sec:ref-cnt-code}

Figure~\ref{fig:ref_count} shows the rest of the concurrent reference counting algorithm from Section~\ref{sec:ref-cnt}.

\begin{figure}
	\small
	\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,linewidth=.99\columnwidth, xleftmargin=5.0ex,numbers=left]
void atomic_shared_ptr<T>::@\textbf{store}@(const shared_ptr<T>& desired) {
	if (desired.ptr != null) increment(desired);
	auto old_ptr = this->ptr.exchange(desired.ptr);
	if (old_ptr != null) delayed_decrement(old_ptr); } @\label{line:destruct1}@

shard_ptr<T> atomic_shared_ptr<T>::@\textbf{load}@() {
  auto ptr = load_and_increment(addressof(this->ptr));
	return shared_ptr(ptr); }

bool atomic_shared_ptr<T>::@\textbf{compare\_and\_swap}@(
  const shared_ptr<T>& expected, const shared_ptr<T>& desired) { 
  auto ptr, guard = ar.acquire(addressof(desired.ptr));
	if (compare_and_swap(this->ptr, expected.ptr, ptr)) {
    if (ptr) increment(ptr);
		if (expected.ptr) delayed_decrement(expected.ptr); @\label{line:destruct2}@
    ar.release(guard);
		return true;
	} else {
    ar.release(guard);
		return false; } }

snapshot_ptr<T> atomic_shared_ptr<T>::@\textbf{get\_snapshot}@() {
 	auto ptr, guard = ar.try_acquire(addressof(this->ptr));
 	if(guard != @$\bot$@) return snapshot_ptr<T>(ptr, guard);
 	ptr, guard = ar.acquire(addressof(this->ptr));
 	increment(ptr); // increment reference count
 	ar.release(guard);
 	return snapshot_ptr<T>(ptr, @$\bot$@); }

void snapshot_ptr<T>::release() {
  if (this->guard != @$\bot$@) ar.release(this->guard);
  else decrement(this->ptr); }
	\end{lstlisting}
	\caption{Implementation of atomic reference-counted pointers using the generalized acquire-retire interface from Figure~\ref{fig:new-ar-interface}.}
	\label{fig:ref_count}
\end{figure}

==> useability.tex <==

\section{Usability}
\label{sec:usability}


